Instant Loans Can Lift Subjective Well-Being: A Randomized Evaluation of Digital Credit in Nigeria

Digital loans have exploded in popularity across low and middle income countries, providing short term, high interest credit via mobile phones. This paper reports the results of a randomized evaluation of a digital loan product in Nigeria. Being randomly approved for digital credit (irrespective of credit score) substantially increases subjective well-being after an average of three months. For those who are approved, being randomly offered larger loans has an insignificant effect. Neither treatment significantly impacts other measures of welfare. We rule out large short-term impacts either positive or negative: on income and expenditures, resilience, and women's economic empowerment.

==> RF_Tables/Tab_Het_totalever_beforesurvey.tex <==
\begin{table}[H]\renewcommand{\arraystretch}{1.3}\caption{Treatment Effect Heterogeneity: Total Borrowing (Partner FSP)}\label{Tab_het_totalever_beforesurvey}\vspace{3mm}\begin{center}\begin{threeparttable}[H]\begin{tabular}{lcccccc}
\toprule\toprule
{} &          (1) &          (2) &          (3) &          (4) &          (5) \\
\midrule
Auto-approval * Under-threshold                                          &      13896.6 &      12746.6 &      12979.2 &      13519.4 &      18574.0 \\
                                                                         &  (3504.7)*** &  (2439.2)*** &  (2002.1)*** &  (4520.1)*** &  (6466.3)*** \\
Auto-approval * Over-threshold                                           &       1386.4 &       1448.6 &       1380.2 &       1387.5 &       1432.2 \\
                                                                         &     (1482.5) &     (1482.0) &     (1482.1) &     (1482.0) &     (1485.9) \\
Initial Offer                                                            &       1262.2 &       1258.4 &       1275.8 &       1264.4 &       1260.1 \\
                                                                         &   (137.7)*** &   (137.4)*** &   (137.9)*** &   (138.2)*** &   (139.2)*** \\
Auto-approval * Under-threshold * Credit Score                           &     -27032.6 &              &              &              &     -32300.1 \\
                                                                         &    (35233.3) &              &              &              &    (34733.2) \\
Auto-approval * Under-threshold * Unemployed                             &              &      -1447.3 &              &              &      -2520.5 \\
                                                                         &              &     (3607.2) &              &              &     (3603.1) \\
Auto-approval * Under-threshold * Business                               &              &              &      -1897.1 &              &      -3404.4 \\
                                                                         &              &              &     (3957.2) &              &     (3792.6) \\
Auto-approval * Under-threshold * Male                                   &              &              &              &      -1462.3 &      -2556.1 \\
                                                                         &              &              &              &     (4861.5) &     (4854.5) \\
Credit Score                                                             &       6890.2 &       6487.7 &       6958.6 &       6964.5 &       6412.5 \\
                                                                         &   (3408.6)** &    (3426.0)* &   (3409.1)** &   (3400.2)** &    (3437.8)* \\
Unemployed                                                               &      -6797.2 &      -8588.6 &      -7048.6 &      -6785.1 &      -8419.1 \\
                                                                         &  (1382.9)*** &  (1630.2)*** &  (1374.7)*** &  (1390.7)*** &  (1659.5)*** \\
Business                                                                 &       3493.4 &       3572.8 &       4279.5 &       3450.0 &       3985.9 \\
                                                                         &  (1295.5)*** &  (1298.3)*** &  (1497.6)*** &  (1303.1)*** &  (1535.0)*** \\
Male                                                                     &      -4406.4 &      -4294.7 &      -4337.1 &      -4733.0 &      -4550.2 \\
                                                                         &  (1510.4)*** &  (1516.0)*** &  (1519.5)*** &  (1732.0)*** &  (1749.9)*** \\
\midrule
\multirow{1}{3cm}{\footnotesize Mean dep var. (Standard approval group)} &     20036.68 &     20036.68 &     20036.68 &     20036.68 &     20036.68 \\
                                                                         &              &              &              &              &              \\
\footnotesize N                                                          &         1611 &         1611 &         1611 &         1611 &         1611 \\
\bottomrule\bottomrule
\end{tabular}\footnotesize \begin{tablenotes}\item Each column is a separate WLS regression, where we examine heterogeneity in treatment effects. 
The outcome of interest is the total borrowing from the Partner FSP. The credit score ranges from 0-1. 
 Note that in all regressions, 
we also include the under-threshold dummy, and an interaction with the under-threshold dummy and the characteristic of interest. 
These coefficients are not displayed in this table.  Parentheses contain robust standard errors. *p$<$.1, **p$<$.05, ***p$<$.01.
 \end{tablenotes}\end{threeparttable}\end{center}\end{table}

==> RF_Tables/table2_alternate.tex <==
\begin{table}[H]\renewcommand{\arraystretch}{1.3}\caption{Impacts of Digital Credit Access on Welfare Measures}\label{table2_alternate}\vspace{3mm}\begin{center}\begin{threeparttable}[H]\begin{tabular}{lccccccc}
\toprule\toprule
{} &                                                                   (1) &                                                                 (2) &                                                           (3) &                                                                     (4) &                                                    (5) &                                                          (6) &                                                                     (7) \\
&&&\multicolumn{2}{m{2.4cm}}{\centering \small Resilience}&\multicolumn{2}{m{2.4cm}}{\centering \small Women's Economic Empowerment}\\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}
{} & \multicolumn{1}{m{1.7cm}}{\centering \small Total Borrowing from FSP} & \multicolumn{1}{m{1.5cm}}{\centering \small Financial Health Index} & \multicolumn{1}{m{1.5cm}}{\centering \small Resilience Index} & \multicolumn{1}{m{1.7cm}}{\centering \small Financial Resilience Index} & \multicolumn{1}{m{1.0cm}}{\centering \small WEE Index} & \multicolumn{1}{m{1.0cm}}{ \small Financial Index} & \multicolumn{1}{m{1.7cm}}{\centering \small Subjective Wellbeing Index} \\
{} &                    \multicolumn{1}{m{1.7cm}}{\centering \small (NGN)} &                       \multicolumn{1}{m{1.5cm}}{\centering \small } &             \multicolumn{1}{m{1.7cm}}{\centering \small (SD)} &                       \multicolumn{1}{m{1.5cm}}{\centering \small (SD)} &      \multicolumn{1}{m{1.7cm}}{\centering \small (SD)} &            \multicolumn{1}{m{1.7cm}}{\centering \small (SD)} &                       \multicolumn{1}{m{1.5cm}}{\centering \small (SD)} \\
\midrule
\multirow{1}{3cm}{\footnotesize Auto-Approval *Under-threshold}          &                                                               11656.6 &                                                               0.024 &                                                         0.002 &                                                                  -0.069 &                                                  0.343 &                                                       -0.144 &                                                                   0.281 \\
                                                                         &                                                           (1797.0)*** &                                                             (0.018) &                                                       (0.061) &                                                                 (0.096) &                                                (0.220) &                                                     (0.081)* &                                                              (0.106)*** \\
                                                                         &                                                                 [0.0] &                                                             [0.166] &                                                       [0.974] &                                                                 [0.718] &                                                [0.149] &                                                      [0.149] &                                                                 [0.008] \\
\multirow{1}{3cm}{\footnotesize Auto-Approval *Over-threshold}           &                                                                1226.8 &                                                               0.005 &                                                         0.042 &                                                                   0.014 &                                                  0.035 &                                                        0.062 &                                                                  -0.013 \\
                                                                         &                                                              (1476.6) &                                                             (0.008) &                                                       (0.026) &                                                                 (0.046) &                                                (0.095) &                                                      (0.039) &                                                                 (0.049) \\
                                                                         &                                                                 [0.4] &                                                             [0.565] &                                                       [0.200] &                                                                 [0.769] &                                                [0.717] &                                                      [0.214] &                                                                 [0.796] \\
\footnotesize Initial Offer                                              &                                                                1239.0 &                                                               0.001 &                                                        -0.000 &                                                                   0.002 &                                                 -0.002 &                                                       -0.003 &                                                                   0.007 \\
                                                                         &                                                            (136.3)*** &                                                            (0.001)* &                                                       (0.002) &                                                                 (0.004) &                                                (0.009) &                                                      (0.004) &                                                                 (0.004) \\
                                                                         &                                                                 [0.0] &                                                             [0.098] &                                                       [0.868] &                                                                 [0.868] &                                                [0.816] &                                                      [0.664] &                                                                 [0.113] \\
\midrule
\multirow{1}{3cm}{\footnotesize Mean dep var. (Standard approval group)} &                                                             20036.676 &                                                               0.704 &                                                         0.000 &                                                                   0.002 &                                                 -0.003 &                                                       -0.000 &                                                                  -0.002 \\
                                                                         &                                                                       &                                                                     &                                                               &                                                                         &                                                        &                                                              &                                                                         \\
\footnotesize N                                                          &                                                                  1611 &                                                                1611 &                                                          1312 &                                                                    1403 &                                                    757 &                                                         1611 &                                                                    1611 \\
\bottomrule\bottomrule
\end{tabular}\footnotesize \begin{tablenotes}\item Notes: Each column is a separate WLS regression. Each regression controls for respondent gender, education, 
head of the household, ethnicity, location (state), household size, age, and respondent's credit score status (1 = under threshold) at 
the time of enrolment. We include enumerator, and week of enrolment fixed effects. 29 respondents did not report their 
age -- we code these values as 0, and include a dummy variable that controls for these missing values. 
Parentheses contain robust standard errors, and square brackets contain p-values after adjusting for 
multiple hypothesis testing. 
\end{tablenotes}\end{threeparttable}\end{center}\end{table}
